Understanding self-supervised Learning Dynamics without Contrastive Pairs

While contrastive approaches of self-supervised learning (SSL) learn representations by minimizing the distance between two augmented views of the same data point (positive pairs) and maximizing views from different data points (negative pairs), recent \emph{non-contrastive} SSL (e.g., BYOL and SimSiam) show remarkable performance {\it without} negative pairs, with an extra learnable predictor and a stop-gradient operation. A fundamental question arises: why do these methods not collapse into trivial representations? We answer this question via a simple theoretical study and propose a novel approach, DirectPred, that \emph{directly} sets the linear predictor based on the statistics of its inputs, without gradient training. On ImageNet, it performs comparably with more complex two-layer non-linear predictors that employ BatchNorm and outperforms a linear predictor by $2.5\%$ in 300-epoch training (and $5\%$ in 60-epoch). DirectPred is motivated by our theoretical study of the nonlinear learning dynamics of non-contrastive SSL in simple linear networks. Our study yields conceptual insights into how non-contrastive SSL methods learn, how they avoid representational collapse, and how multiple factors, like predictor networks, stop-gradients, exponential moving averages, and weight decay all come into play. Our simple theory recapitulates the results of real-world ablation studies in both STL-10 and ImageNet. Code is released https://github.com/facebookresearch/luckmatters/tree/master/ssl.

==> backup.tex <==
\vspacenoarxiv{-0.1in}
\section{Analysis of BYOL learning}
\vspacenoarxiv{-0.1in}
\label{sec:byol-analysis}
In BYOL, the two networks are no-longer identical and, interestingly, only positive pairs are used for training. The first network with weights $\cW_1 = \cW := \{\cW_\base, \cW_\pred\}$ is an \emph{online} network that is trained to predict the output of the second \emph{target} network with weights $\cW_2 = \cW'$, using a learnable  \emph{predictor} $\cW_{\pred}$ to map the online to target outputs (Fig. \ref{fig:notation}(a) and Fig.~1 in \cite{byol}). In contrast, the target network has $\cW' := \{\cW'_\base\}$, where $\cW'_\base$ is an exponential moving average (EMA) of $\cW_\base$: $\cW_\base'(t+1)  =  \gamma_\ema \cW_\base'(t) + (1-\gamma_\ema)\cW_\base(t)$. Since BYOL only uses positive pairs, we consider the following loss function:
\begin{equation}
\vspace{-0.03in}
    r := \frac{1}{2}\|\vf_L(\vx_1; \cW) - \vf_{L'}(\vx_+; \cW')\|^2_2 
\end{equation}
where the input data are positive pairs: $\vx_1, \vx_+\sim p_\aug(\cdot|\vx)$ and $\vx \sim p(\cdot)$. The two outputs, $\vf_{L}(\vx_1; \cW)$ and $\vf_{L'}(\vx_+; \cW')$, are from the online and the target networks, respectively. Note that $L' < L$ due to the presence of an extra predictor on the side of online network ($\cW$).  % Similar to SimCLR case, we leave the incorporation of $\ell_2$ normalization of the final layer as the future work. 

In this paper, we only analyze the case where there is no EMA (or $\gamma_\ema=0$). Recent works~\cite{chen2020exploring,byol} show that without EMA, things still works reasonably well. We also show it is the case in Tbl.~\ref{tbl:factors-in-byol}. Therefore, we first analyze the case without EMA, which means that $\gamma_\ema = 0$ and thus $\cW_\base{} = \cW'_\base{}$.

We leave EMA case for future work.

\subsection{No predictor}
Without the predictor, $\cW'=\cW$ and the BYOL update without BN is
\begin{equation}
\vec\left(\Delta W_l\right)_\sym = -\eee{\vx}{\var_{\vx'\sim p_\aug(\cdot|\vx)}\left[K_l(\vx')\right]}\vec(W_l) \label{eq:bn-sym-grad}
\end{equation}
(see App.~\ref{sec:derivation-BYOL} for proof). This update only promotes variance minimization in the representations of different augmented views of the same data samples and therefore would yield model collapse. 

\subsection{In the presence of BatchNorm}
We now consider the effects played by the extra predictor and BatchNorm (BN)~\cite{batchnorm} in BYOL. 
Our interest in BatchNorm is motivated by a recent blogpost~\cite{byol-bn-blog}. 
We will see that combining both could yield a sufficient condition to create an implicit contrastive term that could help BYOL learn.  Here we focus on BatchNorm, leaving an analysis of other normalization techniques in nonlinear BYOL settings for future work.  

When adding predictor, Theorem~\ref{thm:l2-two-tower} can still be applied by adding identity layers on top of the target network $\cW'$ so that the online and the target networks have the same depth. Theorem 5 in~\cite{yuandong-relu} demonstrates this version of BN shifts the downward gradients so their mini-batch mean is $\vzero{}$:
\begin{equation}
    \dbtilde\vg^i_l := \vg^i_l - \frac{1}{|B|}\sum_{i\in B}\vg^i_l = \vg^i_l - \bar\vg_l \label{eq:grad-zero-mean}
\end{equation}
Here $\vg_l^i$ is the $i$-th sample in a batch and $\bar\vg_l$ is the batch average (same for $\bar\vf_l$). Backpropagating through this BN (vs. just subtracting the mean only in the forward pass\footnote{In PyTorch, the former is \texttt{x-x.mean()} and the latter is \texttt{x-x.mean().detach()}.}), leads to a correction term:

\iffalse
For this, we make the following assumptions: 
\begin{assumption}
\label{assumption:byol}
The ReLU gating from layer $l$ to $L$ is constant over the batch $B$ given $\cW$ and $\cW'$. 
\end{assumption}
If the network is linear from layer $l$ to the topmost, then this assumption trivially holds. For ReLU networks, in general the gating is piece-wise constant depends on $\vx_i$. For different sample $i$, it might take different values. 
\fi

\begin{theorem}
\label{thm:zero-mean-gradient-update}
If \textbf{(1)} the network is linear from layer $l$ to the topmost and \textbf{(2)} the downward gradient $\vg_l$ undergoes Eqn.~\ref{eq:grad-zero-mean}, then with large batch limits, the correction of the update is\footnote{A formal treatment requires  Jacobian $J$ to incorporate BatchNorm's contribution and is left for future work.} (for brevity, dependency on $\cW$ is omitted, while dependency on $\cW'$ is made explicit): 
\small{
\begin{eqnarray}
    \vec(\bnterm{}) &\!=\!& \eee{\vx}{\bar K_l(\vx)} \eee{\vx}{\bar K_l^\t(\vx)}\vec(W_l) \\
    &\!-\!&  \eee{\vx}{\bar K_l(\vx)} \eee{\vx}{\bar K_l^\t(\vx;\cW')}\vec(W'_{l}) \nonumber
\end{eqnarray}}
and the corrected weight update is $\widetilde{\Delta W_l} := \Delta W_l + \bnterm{}$. Using Eqn.~\ref{eq:bn-sym-grad}, we have:
{\small
\begin{eqnarray}
    \vec(\widetilde{\Delta W_l}) &\!=\!& \vec(\Delta W_l)_\sym -
    \var_{\vx}\left[\bar K_l(\vx)\right]\vec(W_l) \nonumber \\
    &\!+\!& \Cov_{\vx}\left[\bar K_l(\vx), \bar K_l(\vx;\cW')\right]\vec(W'_l)\label{eq:corrected-gradient-byol}
\end{eqnarray}}
\end{theorem}
\begin{corollary}[SimCLR]
\label{col:bn-simclr}
For SimCLR with contrastive losses $\lsimple$, $\ltriplet$ and $\lnce$, $\bnterm{} = 0$.
\end{corollary}

In BYOL when the predictor is present, $\cW' \neq \cW$ and BN is present, from the analysis above we know that $\bnterm{} \neq 0$, which provides an implicit contrastive term. Note that $\cW' \neq \cW$ means there is a predictor, the online network uses EMA, or both. We first discuss the case without EMA.  

From Theorem~\ref{thm:zero-mean-gradient-update}, if we further consider a single linear predictor, then the following holds. Here $\bar K_{l,\base}(\vx) := \bar K_l(\vx; \cW_\base)$ is the augmentation-mean connection (and only depends on augmented data point $\vx$), and $\hat K_l(\vx) := \bar K_l(\vx) - \eee{\vx}{\bar K_l(\vx)}$ is its zero-mean version.
\begin{corollary}[The role of a predictor in BYOL]
\label{col:bn-byol-no-ema}
If $\cW_\pred = \{W_\pred\}$ is linear and no EMA, then the gradient update $\vec(\widetilde{\Delta W_l})$ is:
{\small
\begin{equation}
    \vec(\Delta W_l)_\sym + \eee{\vx}{\hat K_{l,\base}(\vx) W^\t_\pred (I-W_\pred)\hat K^\t_{l,\base}(\vx)}\vec(W_l).
\end{equation}}
Without stop gradient, the gradient update $\vec(\doublewidetilde{\Delta W_l})$ is:
\begin{equation}
    2\vec(\Delta W_l)_\sym - \var_\vx\left[\bar K_{l,\base}(\vx) (I-W_\pred)^\t\right]\vec(W_l)
\end{equation} 
\end{corollary}

\emph{The Predictor}. To see why $\cW_\pred$ plays a critical role, we check some special case. If $W_\pred = \beta I_{n_L\times n_L}$ ($W_\pred$ has to be a squared matrix), then $\vec(\Delta W_l) = \vec(\Delta W_l)_\sym + \beta(1-\beta) \var_\vx\left[\bar K_{l,\base}(\vx)\right]\vec(W_l)$. If $0 < \beta < 1$, then $\beta(1 - \beta) > 0$ and the covariance operator appears. 
In this regime, BYOL works like SimCLR, \emph{except that} it also minimizes variance across different augmented views of the same data sample through $\vec(\Delta W_l)_\sym$ (Eqn.~\ref{eq:bn-sym-grad}), the first term in Eqn.~\ref{eq:corrected-gradient-byol}. 

Indeed, the recent blogpost~\cite{byol-bn-blog} as well as our own experiments (Tbl.~\ref{tbl:factors-in-byol}) suggests that standard BYOL without BN fails. In addition, we also initialize the predictor with small positive weights (See Appendix~\ref{sec:additional-exp}), and reinitialize the predictor weights once in a while (Tbl.~\ref{tab:reinit}), and BYOL still works, consistent with our theoretical prediction.  

\emph{Stop Gradient}. In BYOL, the target network $\cW'$ serves as a target to be learned from, but does not contribute gradients to the current weight $\cW$. Without EMA, we might wonder whether the target network should also contribute the gradient or not. Corollary~\ref{col:bn-byol-no-ema} shows that this won't work: no matter what $W_\pred$ is, the update always contains a (weighted) \emph{negative} covariance operator. This is shown empirically in~\cite{chen2020exploring}.

\subsection{BYOL without BatchNorm} 
As pointed out by~\cite{byol-without-bn}, BYOL can still work using other normalization techniques that do not rely on cross batch statistics, e.g., GroupNorm~\cite{wu2018group}, Weight Standardization~\cite{weightstandardization} and careful initialization of affine transform of activations. 

Why that's the case? We suspect that this is due to the fact that the additional normalization yields $\eee{\vx}{\bar K_l(\vx)} = 0$ and thus $\vec(\Delta W_l)$ takes the form of Eqn.~\ref{eq:corrected-gradient-byol} no matter whether we have BatchNorm or not, since the correction term $\bnterm{} = 0$. 

In Appendix \ref{sec:exactsolbyol} we derive exact solutions to BYOL for linear architectures without any normalization, to provide conceptual insights into how BYOL can still learn {\it without} contrastive terms, at least in the linear setting.

%which then approximately reduces to the analysis for SimCLR.

\iffalse
consider the following linear dynamic system. 
\begin{equation}
    \vw(t+1) - \vw(t) = -\alpha \left[ \vw(t) - (1 - \rho) \vw_\ema(t)\right] \label{eq:weight-recurrent}
\end{equation}
Using $z$-transform, we could compute its two roots:
\begin{equation}
    z_{1,2} = 1 - \frac{1}{2}\left(\lambda + \alpha \pm \sqrt{ (\lambda + \alpha)^2 - 4\alpha\lambda\rho}\right)
\end{equation}
if $\rho < 0$ then $z_2 > 1 > z_1$, and $\vw(t)$ will have exponential growth. 

When will this happen? Consider the asymmetric structure of BYOL. $\cW$ has a predictor while $\cW_\ema$ doesn't have it. 

Note that $\var_{\vx}\left[\bar K_l(\vx;\cW)\right]$ has large eigenvalues on the direction of separating different samples. By left-multiplying Eqn.~\ref{eq:corrected-gradient-byol} with an eigenvector, we arrive at Eqn.~\ref{eq:weight-recurrent} and the conclusion applies [Need more rigorous handling] 
\fi

\iffalse
In conclusion, to make BYOL work, we need BN (or zero-meaned downward gradient), EMA and asymmetric weights (predictor) at the same time. 

\textbf{Improving BYOL with D2L2}. Based on the analysis, we want the predictor in $\cW$ to have both small and random Jacobians. We want small Jacobians to make $\rho < 0$ happen more often and random Jacobians to ensure all low-level features are trained with equal opportunity. So we propose \emph{Diversity-driven Latent Learning} (D2L2): we reinitialize the predictor once in every $T$ epochs to encourage diversity of the learned representation, and we re-initialize the weights in the predictor by a uniform distribution with a smaller covariance than regular Xavier (or Kaiming) initialization. 
\fi

\iffalse
\begin{tabular}{|c||c|c|c|}
    $\rho_{\mu\nu}$  & Initial & 1 epoch &  20 epochs \\
    \hline
    $\sim [0.7,1]$ & 0.66 & 0.82 & 0.84 \\ 
    $\sim [0.8,1]$ & 0.78 & 0.89 & 0.90 \\ 
    $\sim [0.9,1]$ & 0.90 & 0.95 & 0.95
\end{tabular}
\fi

\begin{table}[h!]
\centering
\caption{\small Top-1 STL performance with different combination of predictor (\textbf{P}), EMA and BatchNorm using BYOL. EMA means $\gamma_\ema = 0.996$. Batch size is 128 and all experiments run on 5 seeds and 100 epochs.}
\label{tbl:factors-in-byol}
\small
\setlength{\tabcolsep}{1.8pt}
\begin{tabular}{|c|c|c|c|}
    - & EMA & BN & EMA, BN \\
    \hline
    $38.7\pm 0.6$ & $39.3\pm 0.9$ & $33.0\pm 0.3$ & $32.8\pm 0.5$
\end{tabular}
$\quad$
\begin{tabular}{|c|c|c|c|c|}
    P & P, EMA & P, BN & P, EMA, BN \\
    \hline
    $39.5\pm 3.1$ & $44.4\pm 3.2$ & $63.6\pm 1.06$ & $\textbf{78.1}\pm 0.3$
\end{tabular}
\end{table}

\begin{table*}[h!]
\centering
\caption{\small Top-1 STL performance using different BatchNorm components in the predictor and the projector of BYOL ($\gamma_\ema=0.996$, $100$ epochs). There is no affine part. ``$\mu$'' = zero-mean normalization only, ``$\mu,\sigma$'' = BN without affine, ``$\mu,\sigma^\nparallel$'' = normalization with mean and std but only backpropagating through mean. All variants with detached zero-mean normalization (in {\color{red} red}) yield similar poor performance as no normalization.}
\label{tbl:factors-in-bn}
\small
\setlength{\tabcolsep}{1.8pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    - & $\mu$ & $\sigma$ & $\mu,\sigma$ & $\mu^\nparallel$ & $\sigma^\nparallel$ & $\mu^\nparallel,\sigma$ & $\mu,\sigma^\nparallel$ & $\mu^\nparallel,\sigma^\nparallel$ \\
     \hline
    $43.9\pm 4.2$ & $64.8\pm 0.6$ & $72.2 \pm 0.9$ & $\textbf{78.1}\pm 0.3$ & ${\color{red} 44.2}\pm 7.0$ & $54.2\pm 0.6$ & ${\color{red} 48.3}\pm 2.7$ & $76.3\pm 0.4$ & ${ \color{red} 47.0}\pm 8.1$ 
\end{tabular}
\end{table*}

\begin{table*}[h!]
    \centering
    \small
    \vspace{-0.1in}
    \caption{\small Top-1 performance of BYOL using reinitialization of the predictor every $T$ epochs.}
    \begin{tabular}{|c||c||c|c|c|}
                         & Original BYOL & ReInit $T=5$ & ReInit $T=10$ & ReInit $T=20$ \\
    \hline
    STL-10 (100 epochs)  &  78.1 &  78.6 & \textbf{79.1} & 79.0 \\
    ImageNet (60 epochs) &  60.9 &  61.9 & \textbf{62.4} & \textbf{62.4} 
    \end{tabular}
    \label{tab:reinit}
\end{table*}

\textbf{Factors underlying BYOL performance}. To test our theory, we perform an ablation study of BYOL on STL-10 by modifying three key components: predictor, EMA and BN. Tbl.~\ref{tbl:factors-in-byol} shows that BN and predictor are important and EMA further improves the performance. First, without a predictor, neither BN nor EMA give good performance. A predictor without BN still doesn't work. A predictor with BN starts to show good performance ($63.6\%$) and further adding EMA leads to the best performance ($78.1\%$). This is consistent with our theoretical findings in Sec.~\ref{sec:byol-analysis}, in which we show that using a predictor with BN yields $\bnterm{} \neq 0$ and leads to an implicit contrastive term. 

To further test our understanding of the role played by BN, we fractionate BN into several sub-components: subtract by batch mean (\texttt{mean-norm}), divide by batch standard deviation (\texttt{std-norm}) and \texttt{affine}, and do ablation studies (Tbl.~\ref{tbl:factors-in-bn}). Surprisingly, removing \texttt{affine} yields slightly better performance on STL-10 (from 78.1\% to 78.7\%). 
We also find that variants of \texttt{mean-norm} performs reasonably, while variants of \emph{detached} \texttt{mean-norm} has similar poor performance as no normalization, supporting that centralizing backpropagated gradient leads to implicit contrastive terms (Sec.~\ref{sec:byol-analysis}). Note that \texttt{std-norm} also helps, which we leave for future analysis. 

We also check whether the online network requires an ``optimal predictor'' as suggested by recent version (v3) of BYOL. For this, we  reinitialize the predictor (\texttt{ReInit}) every $T$ epochs and compare the final performance under linear evaluation protocol. Interestingly, as shown in Tbl.~\ref{tab:reinit}, \texttt{ReInit} actually improves the performance a bit, compared to the original BYOL that keeps training the same predictor, which should therefore be closer to optimal.  Moreover, if we shrink the initial weight range of the predictor to make $\Cov_{\vx}\left[\bar K_l(\vx), \bar K_l(\vx;\cW')\right]$ (third term in Eqn.~\ref{eq:corrected-gradient-byol}) more dominant, and reduce the learning rate, the performance further improves (See Tbl.~\ref{tab:pe} in Appendix~\ref{sec:additional-exp}), thereby corroborating our analysis.  


